Breaking Language Barriers in Visual Language Models via Multilingual Textual Regularization

Rapid advancements in Visual Language Models (VLMs) have transformed multimodal understanding but are often constrained by generating English responses regardless of the input language. This phenomenon has been termed as Image-induced Fidelity Loss (IFL) and stems from limited multimodal multilingual training data. To address this, we propose a continuous multilingual integration strategy that injects text-only multilingual data during visual instruction tuning, preserving the language model's original multilingual capabilities. Extensive evaluations demonstrate that our approach significantly improves linguistic fidelity across languages without degradation in visual performance. We also explore model merging, which improves language fidelity but comes at the cost of visual performance. In contrast, our core method achieves robust multilingual alignment without trade-offs, offering a scalable and effective path to mitigating IFL for global VLM adoption.

==> sections/APP4_evaluating_evaluators.tex <==
Even though we have implemented measures for robustness (such as using different generation configurations for the LLM-as-a-judge evaluators and requiring evaluators to provide summaries to justify their scores) we aim to further ensure the fairness of the provided scores by evaluating them against the reference captions in the dataset.

\subsection{Language Consistency Evaluator Evaluation}

To assess the reliability of the language consistency evaluator model (\textbf{Meta-Llama-3.1-8B-Instruct}), we scored the reference captions from the dataset using the same evaluation process applied to the captions generated by our models.

The dataset provides between 1 to 3 reference captions per image. For this evaluation, we used a single generation configuration (configuration B in Table \ref{tab:parameters_text_llm_as_a_judge}) to ensure consistency.

After scoring all available references for each image, we applied the previously established method to aggregate scores: averaging numerical values and using majority voting with a False fallback for boolean values.\\


\textbf{PUT EVALAUTOR SCORES}\\

As shown, the obtained scores are \textbf{nearly perfect}, demonstrating the effectiveness of the chosen model as an evaluator. However, some minor errors are present, which can be attributed to \textbf{multilingual limitations}. Meta-Llama-3.1-8B-Instruct officially supports seven languages in addition to English (French, German, Hindi, Italian, Portuguese, Spanish, and Thai). While this allows it to handle most European languages, it is expected that the model may occasionally struggle with languages outside its primary training set, leading to some misclassifications.

To mitigate this, we have ensured the use of glotLid to classify the language of each sentence accurately. The primary role of this evaluator model has been to \textbf{assess language consistency}, rather than language identification itself. Since words that deviate from the target language tend to appear in English, which is the main language of the evaluator, the model remains effective in detecting inconsistencies, even if it may not fully recognize all languages.


\subsection{Visual Score Evaluator Evaluation}

To assess whether Qwen2.5-VL-7B-Instruct is an appropriate choice as a visual evaluator, we evaluated its performance using the provided reference captions. By doing so, we ensure that the model fairly assesses captions that are considered correct by human annotators.

Since each image in the dataset is associated with multiple reference captions, we evaluated each caption separately and then aggregated the scores for each image. This approach allows us to analyze how consistently the evaluator assigns high scores to captions that are expected to be accurate.

For this evaluation, we again used a single configuration to generate scores (configuration B on Table \ref{tab:parameters_visual_LLM_as_a_judge}), ensuring a balanced assessment.

And we have followed the same aggregation methodology as we have done until now: mean values for numerical scores and majority voting with False fallback for boolean scores.\\

\textbf{PUT SCORES HERE}\\


As shown in \textbf{FILL}, the obtained scores are acceptable, with reference captions achieving over 80\% acceptability in most cases. Given the subjectivity of image description and the fact that Qwen2.5-VL-7B-Instruct has lower familiarity with certain tested languages, these results confirm that the model is sufficiently reliable as a visual evaluator. While some minor discrepancies may arise due to language variations or different valid interpretations of an image, the overall performance demonstrates that Qwen2.5-VL-7B-Instruct is a suitable choice for evaluating the quality of generated captions.

==> tables/hparams.tex <==
\begin{table*}[ht!]
    \centering
    % \scriptsize
    \footnotesize
    \begin{tabular}{llcccc}    \toprule
        & & \textbf{Stage-1} & \textbf{Stage-1.5} & \textbf{Stage-2} & \textbf{OneVision} \\
        \midrule
        %------------------- VISION ROW -----------------------
        \multicolumn{2}{l}{%
  \begin{tabular}{ll}
    \rotatebox[origin=c]{90}{\textbf{Vision}} & 
    \begin{tabular}{@{}l@{}}
      \textbf{Resolution} \\
      \# Tokens
    \end{tabular}
  \end{tabular}%
} &


    \begin{tabular}{@{}l@{}}
      384 \\
      729
    \end{tabular}
        & \begin{tabular}{@{}c@{}}
      % 384 \(\times \{2\times2, 1\times\{2,3\}, {2,3}\times1\}\)
      AnyRes Max 5 \\
      Max \(729\times5\)
    \end{tabular}
        & \begin{tabular}{@{}c@{}}
      % 384 \(\times\{ \{1\times1\}, ... , \{6\times6\}\}\) 
      AnyRes Max 9\\
      Max \(729\times10\)
    \end{tabular}
        & \begin{tabular}{@{}c@{}}
      % 384 \(\times\{ \{1\times1\}, ... , \{6\times6\}\}\)
      AnyRes Max 9\\
      Max \(729\times10\)
    \end{tabular} \\
        \midrule
        %------------------- DATA ROW -------------------------
        \multicolumn{2}{l}{%
  \begin{tabular}{ll}
    \rotatebox[origin=c]{90}{\textbf{Data}} & 
    \begin{tabular}{@{}l@{}}
      \textbf{Dataset} \\
      \# Vision Samples
    \end{tabular}
  \end{tabular}%
} &
    \begin{tabular}{@{}c@{}}
      Single-Image \\
      558K
    \end{tabular}
        & \begin{tabular}{@{}c@{}}
      Single-Image \\
      3.8M
    \end{tabular}
        & \begin{tabular}{@{}c@{}}
      Single-Image \\
      3.1M
    \end{tabular}
        & \begin{tabular}{@{}c@{}}
      Single/Multi-Image, Video \\
      1.6M
    \end{tabular} \\
        \midrule

%------------------- MODEL ROW -------------------------
        \multicolumn{2}{l}{%
  \begin{tabular}{cc}
    \rotatebox[origin=c]{90}{\textbf{Model}} & 
    \begin{tabular}{@{}l@{}}
      \textbf{Trainable} \\
      7.8B LLM
    \end{tabular}
  \end{tabular}%
} &
    \begin{tabular}{@{}c@{}}
      Projector \\
      20.0M
    \end{tabular}
        & \begin{tabular}{@{}c@{}}
      Full Model \\
      8.2B
    \end{tabular}
        & \begin{tabular}{@{}c@{}}
      Full Model \\
      8.2B
    \end{tabular}
        & \begin{tabular}{@{}c@{}}
      Full Model \\
      8.2B
    \end{tabular} \\
        \midrule

    %------------------- TRAINING ROW -------------------------
        \multicolumn{2}{l}{%
  \begin{tabular}{cc}
    \rotatebox[origin=c]{90}{\textbf{Training}} & 
    \begin{tabular}{@{}l@{}l@{}l@{}}
      \textbf{Batch Size} \\
      \textbf{LR: $\psi_{vision}$} \\
      \textbf{LR: \{$\theta_{proj}, \phi_{LLM}$\}} \\
      Epoch \\
      Warmup Ratio \\
      LR Scheduler \\
      Grad. Accum. \\
    \end{tabular}
  \end{tabular}%
} &
    \begin{tabular}{@{}c@{}}
      128 \\
      \(1\times10^{-3}\) \\
      \(1\times10^{-3}\) \\
      1 \\
      0.03 \\
      Cosine \\
      1 \\
    \end{tabular}
        & \begin{tabular}{@{}c@{}}
      64 \\
      \(2\times10^{-6}\) \\
      \(1\times10^{-5}\) \\
      1 \\
      0.03 \\
      Cosine \\
      2 \\
    \end{tabular}
        & \begin{tabular}{@{}c@{}}
      64 \\
      \(2\times10^{-6}\) \\
      \(1\times10^{-5}\) \\
      1 \\
      0.03 \\
      Cosine \\
      2 \\
    \end{tabular}
        & \begin{tabular}{@{}c@{}}
      64 \\
      \(2\times10^{-6}\) \\
      \(1\times10^{-5}\) \\
      1 \\
      0.03 \\
      Cosine \\
      2 \\
    \end{tabular} \\

        \bottomrule
    \end{tabular}
    \caption{Detailed configuration for each training stage of the LLaVA-OneVision model. For a detailed explanation of AnyRes Max, refer to \citep{llavaonevision}. Anyres Max 5: 384 \(\times \{2\times2, 1\times\{2,3\}, {2,3}\times1\}\). AnyRes Max 9: 384 \(\times\{ \{1\times1\}, ... , \{6\times6\}\}\).}
    \label{tab:onevision-stages}
\end{table*}
